Democratizing Domain-Specific Computing

In the past few years, domain-specific accelerators (DSAs), such as Google's Tensor Processing Units, have shown to offer significant performance and energy efficiency over general-purpose CPUs. An important question is whether typical software developers can design and implement their own customized DSAs, with affordability and efficiency, to accelerate their applications. This article presents our answer to this question.

==> codes/cnn-merlin.tex <==
\begin{lstlisting}[caption=CNN Code Snippet in Merlin C\label{code:cnn_merlin}]
void CnnKernel(
	const float input[NumIn][InImSize][InImSize],
	const float weight[NumOut][NumIn][kKernel][kKernel], 
	const float bias[NumOut], float output[NumOut][OutImSize][OutImSize]) {

  float C[ParallelOut][ImSize][ImSize];
  for (int i = 0; i < NumOut/ParallelOut; i++) {
    // Initialization
	  for (int h = 0; h < ImSize; ++h) {
#pragma ACCEL parallel factor=4
	    for (int w = 0; w < ImSize; ++w){
	      for (int po = 0; po < ParallelOut; po++)
		        C[po][h][w] = 0.f; } }
    // Convolution
#pragma ACCEL pipeline
	  for (int j = 0; j < NumIn; ++j) {
	    for (int h = 0; h < ImSize; ++h) {
#pragma ACCEL parallel factor=4
#pragma ACCEL pipeline FLATTEN  // Pipeline mode fg
	      for (int w = 0; w < ImSize; ++w) {
		      for (int po = 0; po < ParallelOut; po++){
		        float tmp = 0;
			      for (int p = 0; p < kKernel; ++p) {	 
			        for (int q = 0; q < kKernel; ++q){ tmp += ... } }
			      C[po][h][w] += tmp; } } } }
    // Skip ReLU + Max Pooling for brevity
} } 
\end{lstlisting}


% for (int h = 0; h < OutImSize; ++h) {
%        for (int w = 0; w < OutImSize; ++w) {
% 	       for (int po = 0; po < ParallelOut; po++){
% 	         output[(i<<shift)+po][h][w] = ...

==> codes/merlin.tex <==
\begin{lstlisting}[language=C,caption=Merlin Compiler for FPGAs\label{code:merlin}] 
#pragma ACCEL parallel factor = 16
for (int i = 0; i < N; i++) {
    c[i] += a[i] * b[i]; }
\end{lstlisting}

==> figures/cnn-arch-optimized.tex <==
\begin{figure}[!htb]
	\centering
	\includegraphics[width=\linewidth]{figures/sources/cnn-arch-optimized.pdf} 
	\caption{The optimized micro-architecture of the CNN code after resolving the performance bottlenecks.}
	\label{fig:cnn-arch-optimized}
\end{figure}

==> figures/cnn-arch.tex <==
\begin{figure}[!htb]
	\centering
	\includegraphics[width=\linewidth]{figures/sources/cnn-arch.pdf} 
	\caption{The Micro-architecture of the Code Snippet in Code~\ref{code:cnn_hls}}
	\label{fig:cnn-arch}
\end{figure}
